Safety Concerns and Mitigation Approaches Regarding the Use of Deep Learning in Safety-Critical Perception Tasks

Deep learning methods are widely regarded as indispensable when it comes to designing perception pipelines for autonomous agents such as robots, drones or automated vehicles. The main reasons, however, for deep learning not being used for autonomous agents at large scale already are safety concerns. Deep learning approaches typically exhibit a black-box behavior which makes it hard for them to be evaluated with respect to safety-critical aspects. While there have been some work on safety in deep learning, most papers typically focus on high-level safety concerns. In this work, we seek to dive into the safety concerns of deep learning methods and present a concise enumeration on a deeply technical level. Additionally, we present extensive discussions on possible mitigation methods and give an outlook regarding what mitigation methods are still missing in order to facilitate an argumentation for the safety of a deep learning method.

==> concerns.tex <==
\begin{tikzpicture}
	% --- SC1 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (0, -2.5) {};
	\node[align=center, anchor=north] at (0, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc1}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (0, -5) {Data distribution is not a good approximation to real world
	};
	
	% --- SC2 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (2.5, -2.5) {};
	\node[align=center, anchor=north] at (2.5, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc2}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (2.5, -5) {Test data is present in training data		
	};

	% --- SC3 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (5, -2.5) {};
	\node[align=center, anchor=north] at (5, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc3}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (5, -5) {Dependence on labeling quality
	};

	% --- SC4 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (7.5, -2.5) {};
	\node[align=center, anchor=north] at (7.5, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc4}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (7.5, -5) {Distributional shift over time
	};

	% --- SC5 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (10, -2.5) {};
	\node[align=center, anchor=north] at (10, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc5}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (10, -5) {Unknown behavior in rare critical situations
	};

	% --- SC6 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (12.5, -2.5) {};
	\node[align=center, anchor=north] at (12.5, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc6}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (12.5, -5) {Brittleness of ML algorithms
	};

	% --- SC7 ---%
	\node[draw, rounded corners=10pt, text width=2cm, minimum height=6.5cm, fill=gray!10] at (15, -2.5) {};
	\node[align=center, anchor=north] at (15, 0) {
		\includegraphics[width=0.11\textwidth]{imgs/sc7}
	};
	\node[anchor=south, align=center, text width=1.8cm] at (15, -5) {Unreliable confidence information
	};
\end{tikzpicture}

==> insufficiencies.tex <==
The ISO PAS 21448 focuses on safety-critical systems which require a proper situational awareness typically derived from complex sensors and processing algorithms. According to this standard, \ac{SOTIF} is the absence of unreasonable risk due to hazards resulting from functional insufficiencies of the intended functionality (or from reasonably foreseeable misuse by persons). 

safety rely on corect output

While the aim of an \ac{ML} algorithm is to approximate the distribution of data representations in the real world, the concerns described in the previous section can lead to an insufficient approximation.
Consequently, functional insufficiencies are inherent in the algorithm leading to an insufficient performance or robustness with respect to certain inputs the algorithm is facing. As a result, the algorithm can produce erroneous output.

While many concerns leading directly to insufficiencies in the algorithm, some of the concerns rather lead to difficulties with respect to arguing its safety.
In order to reach an acceptable low level of risk, the standard describes an iterative process to identify and evaluate triggering events which could lead to a hazardous behavior of the system. However, identifying such events or arguing their absence becomes quite hard for \acp{NN} due to their black-box character (safety concern explainability). 



%concerns lead to
%an insufficient approximation can lead to insufficent perfomance and robustness, respectively prodicing errounous output.
%
%in addition SOTIF requires to systematically search triggering events. This is very difficult due to lack of explainability etc
%
%
%
%	For some systems, which rely on sensing the external or internal environment, there can be potentially hazardous behavior caused by the intended functionality or performance limitation of a system that is free from the faults addressed in ISO26262. Examples of such limitations include:
%• The inability of the function to correctly comprehend the situation and operate safely; this also includes functions that use machine learning algorithms
%• Insufficient robustness of the function with respect to sensor input variations or diverse environmental conditions

